Symplectic Neural Networks Based on Dynamical Systems

We present and analyze a framework for designing symplectic neural networks (SympNets) based on geometric integrators for Hamiltonian differential equations. The SympNets are universal approximators in the space of Hamiltonian diffeomorphisms, interpretable and have a non-vanishing gradient property. We also give a representation theory for linear systems, meaning the proposed P-SympNets can exactly parameterize any symplectic map corresponding to quadratic Hamiltonians. Extensive numerical tests demonstrate increased expressiveness and accuracy -- often several orders of magnitude better -- for lower training cost over existing architectures. Lastly, we show how to perform symbolic Hamiltonian regression with SympNets for polynomial systems using backward error analysis.

==> jmlr-coverletter-1.0/jmlr_coverletter.tex <==
% !TEX program = pdflatex
\input{jmlr_coverletter_preamble.tex}

\begin{document}
\hfill{\today}

Journal of Machine Learning Research 
 
\bigskip
   
Dear Editors: 

We are writing to submit our manuscript ``{Symplectic Neural Networks Based on Dynamical Systems}'' to the \emph{Journal of Machine Learning Research}.

Our manuscript studies the design, theory and implementation of a class of structure-preserving neural networks that are intrinsically symplectic. The paper develops a novel framework for symplectic neural networks (also known as SympNets or Hamiltonian neural networks) and aims to unify other existing architectures using theory from dynamical systems and Hamiltonian mechanics. 

We suggest the following action editors and referees for our submission.
 
Action Editors:
\begin{itemize}
    \item {Maxim Raginsky, University of Illinois at Urbana-Champaign (maxim@illinois.edu)}
    \item {Stephan Mandt, University of California (mandt@uci.edu)}
    \item {Michael Mahoney, UC Berkeley (mmahoney@stat.berkeley.edu)}
    \item {Jianfeng Lu, Duke University (jianfeng@math.duke.edu)}
\end{itemize}

Reviewers:
\begin{itemize}
    \item {Christian Offen, Universität Paderborn (christian.offen@uni-paderborn.de)}
    \item {Sina Ober-Blöbaum, Universität Paderborn (sinaober@math.uni-paderborn.de)}
    \item {Zhen Zhang, Brown university (zhen\_zhang1@brown.edu)}
    \item {Yifa Tang, Chinese Academy of Sciences (tyf@lsec.cc.ac.cn)}
    \item {Aiqing Zhu, National University of Singapore (zaq@nus.edu.sg)}
\end{itemize}

Our submission has the following keywords: {Structure-preserving Neural Networks}, {Symplectic Neural Networks} {Hamiltonian Neural Networks}, {Dynamical Systems}, {Physics-Informed Machine Learning}.

As the corresponding author, I confirm that I do not have a conflict of interest with the action editors and referees I suggest above. 

\bigskip

Sincerely,

\medskip

Benjamin K Tapley (SINTEF Digital)\\

\end{document}







































